Fine-Grained Classification via Mixture of Deep Convolutional Neural Networks

We present a novel deep convolutional neural network (DCNN) system for fine-grained image classification, called a mixture of DCNNs (MixDCNN). The fine-grained image classification problem is characterised by large intra-class variations and small inter-class variations. To overcome these problems our proposed MixDCNN system partitions images into K subsets of similar images and learns an expert DCNN for each subset. The output from each of the K DCNNs is combined to form a single classification decision. In contrast to previous techniques, we provide a formulation to perform joint end-to-end training of the K DCNNs simultaneously. Extensive experiments, on three datasets using two network structures (AlexNet and GoogLeNet), show that the proposed MixDCNN system consistently outperforms other methods. It provides a relative improvement of 12.7% and achieves state-of-the-art results on two datasets.

==> related_work.tex <==
\section{Background}
\label{sec:related_work}

\subsection{Gaussian Mixture Models}
\label{gmm}
The probability of an image generated by mixture DCNN components is partially similar to the occupation probability of Gaussian Mixture Model (GMM).
In this part we briefly review the occupation probability of a mixture model.
%AB -> ZG: note sure if you need this: "In the GMM parts-based approach to image classification the distribution of local features from images is modelled by a GMM."
A GMM is a generative model comprised of $K$ Gaussian components. 
%AB -> ZG: I personally think you should use k and K for components as it gets confused with classes
Probability of one image $I$ can be represented as,
\begin{equation}
Pr(I|\Theta) = \prod_{c=1}^{C}\sum_{k=1}^{K}\omega_{k}N[o^{k}|\mu_{k},\Sigma_{k}]
\end{equation}
%AB -> ZG: what is O and o, I'm guessing observation? If image then maybe use I?
where $o$ represents observation of image $I$, $\omega$ is the weight, $\mu$ is the mean, $\Sigma$ is the covariance matrix and $\Theta$ represents model parameters.
The occupation probability $\gamma_{k}$ of the observation $t$ for the $k$ th Gaussian component is given by,
\begin{equation}
\gamma_{k}(o_{t}) = \frac{\omega_{k}N[o_{t}|\mu_{k},\Sigma_{k}]}{\sum_{k=1}^{K}\omega_{k}N[o_{t}|\mu_{k},\Sigma_{k}]}
\end{equation}
%AB -> ZG: you have switched from the superscript k to subscript t?

\subsection{Convolutional Neural Networks}

LeCun et al.~\cite{LeCun89} had proposed convolutional neural network for hand writing digit recognition in the early 90s. 
This type of network is capable of generating useful feature representations by learning low level features in early convolutional layers and accumulating them to high level semantic features in the latter convolutional layers.
Recently,  Krizhevsky et al.~\cite{krizhevsky2012imagenet} achieved impressive performance on the ImageNet recognition challenge by incorporating network extensions including Rectifier Linear units and Dropout regularisation~\cite{srivastava2014dropout}.
%AB -> ZG: Not sure the relevance of describing AlexNet structure here. Are you trying to setup to say we use this same structure for each subset network? If so I think it is better put with our methodology which you already have.
%The network structure of Krizhevsky et al.~\cite{krizhevsky2012imagenet} remains a structure with five convolutional layers ($conv1$ to $conv5$) with two fully-connected layers ($fc6$ and $fc7$) followed by a softmax layer which can be interpreted as a logistic regression process.

\subsection{Ensemble Method for Classification}

An early version of an ensemble network has been proposed by Jacobs et al.~\cite{jacobs1991adaptive}, where they presented a supervised learning system that consists of many subset networks with a gating network. Each subset network learns to handle a part of the training cases. 
This system consists of subset networks with an extra feed-forward gating network to determine weights for each subset networks. The weight has been normalized as,
\begin{equation}
\omega_{c} = \frac{exp(z_{c})}{\sum_{c=1}^{C}exp(z_{c})}
\end{equation}
which effectively computes the \textit{softmax} normalisation for the weighted output $z_i$ of the gating network.
%The final prediction is made by the gating network outputs pluses subset networks.

Hinton et al.~\cite{hinton2014distilling} recently proposed a method to train specialist models, each of which specialist is trained on one subset of data. Each subset data is clustered by computing the confusion matrix, which is calculated by the predictions of a generalist model (trained on the whole dataset with all classes). 
The prediction of a test image is made by calculating KL divergence of between the probability distribution of a specialist model and a generalist model.
 
Our proposed method differs from these ensemble networks in two ways. Firstly, we don't use an external gating network. 
%The main differences between our proposed system to theirs is first we don't use external gating network. 
Second, unlike~\cite{jacobs1991adaptive,hinton2014distilling} each specialist model is trained both independently and then jointly within the ensemble framework. %once through the whole process, our mixture model has a jointly training process in the end. 
